UCD: Unlearning in LLMs via Contrastive Decoding

Machine unlearning aims to remove specific information, e.g. sensitive or undesirable content, from large language models (LLMs) while preserving overall performance. We propose an inference-time unlearning algorithm that uses contrastive decoding, leveraging two auxiliary smaller models, one trained without the forget set and one trained with it, to guide the outputs of the original model using their difference during inference. Our strategy substantially improves the tradeoff between unlearning effectiveness and model utility. We evaluate our approach on two unlearning benchmarks, TOFU and MUSE. Results show notable gains in both forget quality and retained performance in comparison to prior approaches, suggesting that incorporating contrastive decoding can offer an efficient, practical avenue for unlearning concepts in large-scale models.

==> approximate_theorem.tex <==
\section{Approximate Theorem} 

We first want to claim that for any $x$ that is in the retrain set the quantity 
\begin{align}
\log p_1(y \mid x) - \log p_2(y \mid x) 
\end{align}
is almost a constant, where $p_1$ and $p_2$ are the small models. To show this, we can plot the histogram of \(p_1(x) - p_2(x)\) and empirically show that it has a small variance / span. As a result, the additive factor on \({p_{\texttt{big}}}(y | x)\) does not change too much with \(y\) (since it is almost a constant). By the properties of the arg-max sampling or multinomial sampling, we note that 
\begin{align}
{p_{\texttt{big}}}(y | x) \propto \exp({p_{\texttt{big}}}(y | x) - c),
\end{align}
for any constant c. This shows that the model \(p_{\mathrm{big}}\) does not change its behavior for samples in the retain set. 

On the other hand, we want to claim that on the forget set prompts $x$ the gap 
\begin{align}
\log p_1(y \mid x) - \log p_2(y \mid x) 
\end{align}
is large for exactly those \(y\) that we want to suppress in \(p_\mathrm{big}(y \mid x)\). Towards this, we first want to ensure that:
\begin{enumerate}
    \item The variance / spread in $\log p_1(y \mid x) - \log p_2(y \mid x) $ is large, and 
    \item The gap $\log p_1(y \mid x) - \log p_2(y \mid x) $  is aligned with  those tokens $y$ that have high score \(p_{\mathrm{big}}(y)\). 
\end{enumerate}

I can incorporate both of these scenarios under the following assumption:

For any top $K$  tokens,  
\begin{align}
\log p_1(y) - \log p_2(y) \propto \log p_{\mathrm{big}}(y \mid x) - \log p^{\mathrm{clean}}_{\mathrm{big}}(y \mid x)  
\end{align}

Suppose the above assumption holds, then for any \(x\),  exists value of \(\alpha_x\) such that our update (with that value of \(\alpha\)) suppress the tokens that are preferred by \(p_{\mathrm{big}}\) but not by \(p^{\mathrm{clean}}_{\mathrm{big}}\). 



==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak





==> plan.tex <==

\vmscomment{TODO LIST for Vinith: 1. Section 5 writing and plots
2. Section 6 writing and plots
3. Difference correlation analysis for approximation assumption, 4. Section 7, 5. Figure 1 -- visualization of contrastive decoding, 6. Appendix
    1. Sampling plots for TOFU
    2. Table with Probability, ROUGE-L, and Truth Ratio for TOFU
    3. Example Generations
        1. TOFU 10%
}


==> problem_setup.tex <==
\paragraph{Gradient Ascent (GA)} A common unlearning baseline, GA maximizes the next-token prediction loss on the forget set to reverse learning on those examples: \begin{equation*} \mathcal{L}{\texttt{GA}} = \mathbb{E}{x\sim\mathcal{D}_{\texttt{forget}}}[\log(\pi(y|x))] \end{equation*} While simple and direct, GA often serves as the foundation for more stable and effective variants.

\paragraph{Gradient Difference (GD)} Extends GA by adding a standard training loss on the retain set to preserve performance: \begin{equation*} \mathcal{L}{\texttt{GD}} = -\mathbb{E}{x\sim\mathcal{D}{\texttt{forget}}}[\log(\pi(y|x))] + \mathbb{E}{x\sim\mathcal{D}_{\texttt{retain}}}[\log(\pi(y|x))]
\end{equation*}

\paragraph{KL Regularization} Adds a KL term to control divergence between the updated model and a reference model on either the forget or retain set: \begin{equation*} \mathcal{L}{\texttt{KL}}(\pi,\refmodel) = \mathbb{E}{x\sim\mathcal{D}{\texttt{choice}}}[D{\texttt{KL}}(\pi(y|x)|\refmodel(y|x))], \quad \texttt{choice} \in {\texttt{forget}, \texttt{retain}} \end{equation*} This encourages forgetting via divergence on $\mathcal{D}{\texttt{forget}}$ or stability via alignment on $\mathcal{D}{\texttt{retain}}$.

\paragraph{Preference Optimization (PO)} Optimizes for refusal-like or random responses on the forget set while retaining standard performance elsewhere: \begin{equation*} \mathcal{L}{\texttt{PO}} = \mathbb{E}{x\sim\mathcal{D}{\texttt{alt}}}[\log(\pi(y|x))] + \mathbb{E}{x\sim\mathcal{D}{\texttt{retain}}}[\log(\pi(y|x))] \end{equation*} Here, $\mathcal{D}{\texttt{alt}}$ may include modified forget samples with refusal or random targets.

\paragraph{Negative Preference Optimization (NPO)} Adapts Direct Preference Optimization by treating the forget set as a negative-only preference dataset. The resulting objective is: \begin{equation*} \mathcal{L}{\texttt{NPO}} = \frac{2}{\beta}\mathbb{E}{x\sim\mathcal{D}{\texttt{forget}}}\left[\log\left(1 + \left(\frac{\pi{\theta}(y|x)}{\refmodel(y|x)}\right)^{\beta}\right)\right] \end{equation*}

==> qjbrrrnydnfnmpfdqhfjznfbtydkxrnq/approximate_theorem.tex <==
\section{Approximate Theorem} 

We first want to claim that for any $x$ that is in the retrain set the quantity 
\begin{align}
\log p_1(y \mid x) - \log p_2(y \mid x) 
\end{align}
is almost a constant, where $p_1$ and $p_2$ are the small models. To show this, we can plot the histogram of \(p_1(x) - p_2(x)\) and empirically show that it has a small variance / span. As a result, the additive factor on \({p_{\texttt{big}}}(y | x)\) does not change too much with \(y\) (since it is almost a constant). By the properties of the arg-max sampling or multinomial sampling, we note that 
\begin{align}
{p_{\texttt{big}}}(y | x) \propto \exp({p_{\texttt{big}}}(y | x) - c),
\end{align}
for any constant c. This shows that the model \(p_{\mathrm{big}}\) does not change its behavior for samples in the retain set. 

On the other hand, we want to claim that on the forget set prompts $x$ the gap 
\begin{align}
\log p_1(y \mid x) - \log p_2(y \mid x) 
\end{align}
is large for exactly those \(y\) that we want to suppress in \(p_\mathrm{big}(y \mid x)\). Towards this, we first want to ensure that:
\begin{enumerate}
    \item The variance / spread in $\log p_1(y \mid x) - \log p_2(y \mid x) $ is large, and 
    \item The gap $\log p_1(y \mid x) - \log p_2(y \mid x) $  is aligned with  those tokens $y$ that have high score \(p_{\mathrm{big}}(y)\). 
\end{enumerate}

I can incorporate both of these scenarios under the following assumption:

For any top $K$  tokens,  
\begin{align}
\log p_1(y) - \log p_2(y) \propto \log p_{\mathrm{big}}(y \mid x) - \log p^{\mathrm{clean}}_{\mathrm{big}}(y \mid x)  
\end{align}

Suppose the above assumption holds, then for any \(x\),  exists value of \(\alpha_x\) such that our update (with that value of \(\alpha\)) suppress the tokens that are preferred by \(p_{\mathrm{big}}\) but not by \(p^{\mathrm{clean}}_{\mathrm{big}}\). 



==> qjbrrrnydnfnmpfdqhfjznfbtydkxrnq/arxiv_style.tex <==



 \usepackage[letterpaper, left=1in, right=1in, top=1in, bottom=1in]{geometry}

\usepackage[colorlinks=true, linkcolor=blue!70!black, citecolor=blue!70!black]{hyperref}
\usepackage{microtype} 


\usepackage{algorithm}

\usepackage[noend]{algpseudocode} 
\renewcommand{\algorithmicrequire}{\textbf{Input:}} 
\algblockdefx[class]{Class}{EndClass}[1]{\textbf{object} \textsc{#1}:}{\textbf{end object}}
\makeatletter  
\ifthenelse{\equal{\ALG@noend}{t}}%
  {\algtext*{EndClass}} 
  {}%
\makeatother 


\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{amsmath}
\usepackage{bbm}
\usepackage{amsfonts}
\usepackage{amssymb}
\let\vec\undefined
\usepackage{xpatch}
\usepackage{pifont}
\usepackage{array}
\usepackage{booktabs}
\usepackage{blindtext}
\usepackage{caption}


==> qjbrrrnydnfnmpfdqhfjznfbtydkxrnq/forget05_tables.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{lccc}
\toprule
\multicolumn{4}{c}{\textbf{Real World}} \\
\midrule
\textbf{Method} & \textbf{ROUGE~\textuparrow} & \textbf{Prob~\textuparrow} & \textbf{Truth Ratio~\textuparrow} \\
\midrule
\rowcolor{lightgray}  Baseline & 0.923 ± 0.039 & 0.405 ± 0.073 & 0.554 ± 0.068 \\
UCD & 0.875 ± 0.061 & 0.433 ± 0.067 & 0.580 ± 0.079 \\
\rowcolor{lightgray}  UCS & 0.883 ± 0.009 & 0.399 ± 0.004 & 0.514 ± 0.006 \\
Grad Ascent & 0.000 ± 0.000 & 0.247 ± 0.017 & 0.391 ± 0.018 \\
\rowcolor{lightgray}  Grad Diff & 0.487 ± 0.385 & 0.476 ± 0.151 & 0.672 ± 0.116 \\
NPO & 0.727 ± 0.456 & 0.329 ± 0.013 & 0.505 ± 0.030 \\
\rowcolor{lightgray}  NPO + RT & 0.925 ± 0.030 & 0.443 ± 0.112 & 0.608 ± 0.104 \\
\bottomrule
\end{tabular}
\caption{Additional metrics comparing baselines and UCD / UCS on Llama2-13B from TOFU 5\% measuring model utility on the real world QA pairs.}
\end{table}

\begin{table}[h!]
\centering
\begin{tabular}{lccc}
\toprule
\multicolumn{4}{c}{\textbf{Real Authors}} \\
\midrule
\textbf{Method} & \textbf{ROUGE~\textuparrow} & \textbf{Prob~\textuparrow} & \textbf{Truth Ratio~\textuparrow} \\
\midrule
\rowcolor{lightgray}  Baseline & 0.972 ± 0.002 & 0.403 ± 0.084 & 0.541 ± 0.075 \\
UCD & 0.866 ± 0.110 & 0.480 ± 0.069 & 0.620 ± 0.074 \\
\rowcolor{lightgray}  UCS & 0.975 ± 0.002 & 0.395 ± 0.004 & 0.513 ± 0.004 \\
Grad Ascent & 0.000 ± 0.000 & 0.261 ± 0.014 & 0.412 ± 0.060 \\
\rowcolor{lightgray}  Grad Diff & 0.476 ± 0.372 & 0.484 ± 0.144 & 0.661 ± 0.142 \\
NPO & 0.724 ± 0.482 & 0.344 ± 0.024 & 0.511 ± 0.028 \\
\rowcolor{lightgray}  NPO + RT & 0.958 ± 0.031 & 0.434 ± 0.095 & 0.589 ± 0.090 \\
\bottomrule
\end{tabular}
\caption{Additional metrics comparing baselines and UCD / UCS on Llama2-13B from TOFU 5\% measuring model utility on the real author QA pairs.}
\end{table}

\begin{table}[h!]
\centering
\begin{tabular}{lccc}
\toprule
\multicolumn{4}{c}{\textbf{Retrain}} \\
\midrule
\textbf{Method} & \textbf{ROUGE~\textuparrow} & \textbf{Prob~\textuparrow} & \textbf{Truth Ratio~\textuparrow} \\
\midrule
\rowcolor{lightgray}  Baseline & 0.437 ± 0.005 & 0.352 ± 0.141 & 0.361 ± 0.005 \\
UCD & 0.626 ± 0.199 & 0.661 ± 0.346 & 0.491 ± 0.071 \\
\rowcolor{lightgray}  UCS & 0.574 ± 0.005 & 0.604 ± 0.001 & 0.452 ± 0.002 \\
Grad Ascent & 0.000 ± 0.000 & 0.000 ± 0.000 & 0.179 ± 0.022 \\
\rowcolor{lightgray}  Grad Diff & 0.301 ± 0.147 & 0.241 ± 0.161 & 0.366 ± 0.067 \\
NPO & 0.237 ± 0.126 & 0.098 ± 0.046 & 0.309 ± 0.023 \\
\rowcolor{lightgray}  NPO + RT & 0.409 ± 0.026 & 0.283 ± 0.119 & 0.356 ± 0.027 \\
\bottomrule
\end{tabular}
\caption{Additional metrics comparing baselines and UCD / UCS on Llama2-13B from TOFU 5\% measuring model utility on the retain QA pairs.}
\end{table}

\begin{table}[h!]
\centering
\begin{tabular}{lccc}
\toprule
\multicolumn{4}{c}{\textbf{Forget}} \\
\midrule
\textbf{Method} & \textbf{ROUGE~\textuparrow} & \textbf{Prob~\textuparrow} & \textbf{Truth Ratio~\textuparrow} \\
\midrule
\rowcolor{lightgray}  Baseline & 0.400 ± 0.002 & 0.211 ± 0.082 & 0.720 ± 0.004 \\
UCD & 0.340 ± 0.049 & 0.090 ± 0.054 & 0.634 ± 0.036 \\
\rowcolor{lightgray}  UCS & 0.410 ± 0.003 & 0.272 ± 0.003 & 0.666 ± 0.002 \\
Grad Ascent & 0.000 ± 0.000 & 0.000 ± 0.000 & 0.542 ± 0.062 \\
\rowcolor{lightgray}  Grad Diff & 0.001 ± 0.002 & 0.000 ± 0.000 & 0.506 ± 0.180 \\
NPO & 0.234 ± 0.145 & 0.080 ± 0.047 & 0.736 ± 0.027 \\
\rowcolor{lightgray}  NPO + RT & 0.315 ± 0.065 & 0.065 ± 0.024 & 0.705 ± 0.039 \\
\bottomrule
\end{tabular}
\caption{Additional metrics comparing baselines and UCD / UCS on Llama2-13B from TOFU 5\% measuring model utility on the forget QA pairs.}
\end{table}

==> qjbrrrnydnfnmpfdqhfjznfbtydkxrnq/forget10_tables.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{lccc}
\toprule
\multicolumn{4}{c}{\textbf{Real World}} \\
\midrule
\textbf{Method} & \textbf{ROUGE~\textuparrow} & \textbf{Prob~\textuparrow} & \textbf{Truth Ratio~\textuparrow} \\
\midrule
\rowcolor{lightgray} Baseline & 0.931 ± 0.035 & 0.433 ± 0.071 & 0.580 ± 0.067 \\ 
UCD & 0.883 ± 0.007 & 0.465 ± 0.028 & 0.613 ± 0.047 \\
\rowcolor{lightgray}  UCS & 0.906 ± 0.017 & 0.403 ± 0.023 & 0.531 ± 0.034 \\
Grad Ascent & 0.477 ± 0.523 & 0.291 ± 0.040 & 0.348 ± 0.161 \\
\rowcolor{lightgray}  Grad Diff & 0.863 ± 0.058 & 0.563 ± 0.017 & 0.723 ± 0.011 \\
NPO & 0.929 ± 0.020 & 0.415 ± 0.088 & 0.580 ± 0.087 \\
\rowcolor{lightgray}  NPO + RT & 0.896 ± 0.007 & 0.499 ± 0.004 & 0.658 ± 0.005 \\
\bottomrule
\end{tabular}
\caption{Additional metrics comparing baselines and UCD / UCS on Llama2-13B from TOFU 10\% measuring model utility on the real world QA pairs.}
\end{table}

\begin{table}[h!]
\centering
\begin{tabular}{lccc}
\toprule
\multicolumn{4}{c}{\textbf{Real Authors}} \\
\midrule
\textbf{Method} & \textbf{ROUGE~\textuparrow} & \textbf{Prob~\textuparrow} & \textbf{Truth Ratio~\textuparrow} \\
\midrule
\rowcolor{lightgray}  Baseline & 0.973 ± 0.007 & 0.421 ± 0.071 & 0.558 ± 0.066 \\
UCD & 0.961 ± 0.018 & 0.495 ± 0.041 & 0.631 ± 0.048 \\
\rowcolor{lightgray}  UCS & 0.968 ± 0.007 & 0.395 ± 0.046 & 0.515 ± 0.059 \\
Grad Ascent & 0.480 ± 0.526 & 0.284 ± 0.031 & 0.365 ± 0.122 \\
\rowcolor{lightgray}  Grad Diff & 0.796 ± 0.026 & 0.676 ± 0.049 & 0.817 ± 0.050 \\
NPO & 0.972 ± 0.007 & 0.416 ± 0.109 & 0.564 ± 0.095 \\
\rowcolor{lightgray}  NPO + RT & 0.955 ± 0.011 & 0.515 ± 0.008 & 0.654 ± 0.012 \\
\bottomrule
\end{tabular}
\caption{Additional metrics comparing baselines and UCD / UCS on Llama2-13B from TOFU 10\% measuring model utility on the real author QA pairs.}
\end{table}

\begin{table}[h!]
\centering
\begin{tabular}{lccc}
\toprule
\multicolumn{4}{c}{\textbf{Retrain}} \\
\midrule
\textbf{Method} & \textbf{ROUGE~\textuparrow} & \textbf{Prob~\textuparrow} & \textbf{Truth Ratio~\textuparrow} \\
\midrule
\rowcolor{lightgray}  Baseline & 0.413 ± 0.029 & 0.333 ± 0.113 & 0.306 ± 0.067 \\
UCD & 0.539 ± 0.195 & 0.645 ± 0.251 & 0.445 ± 0.012 \\
\rowcolor{lightgray}  UCS & 0.776 ± 0.256 & 0.796 ± 0.240 & 0.461 ± 0.027 \\
Grad Ascent & 0.229 ± 0.246 & 0.080 ± 0.087 & 0.245 ± 0.099 \\
\rowcolor{lightgray}  Grad Diff & 0.339 ± 0.033 & 0.233 ± 0.043 & 0.471 ± 0.028 \\
NPO & 0.379 ± 0.067 & 0.223 ± 0.065 & 0.351 ± 0.033 \\
\rowcolor{lightgray}  NPO + RT & 0.355 ± 0.020 & 0.307 ± 0.005 & 0.371 ± 0.004 \\
\bottomrule
\end{tabular}
\caption{Additional metrics comparing baselines and UCD / UCS on Llama2-13B from TOFU 10\% measuring model utility on the retain QA pairs.}
\end{table}

\begin{table}[h!]
\centering
\begin{tabular}{lccc}
\toprule
\multicolumn{4}{c}{\textbf{Forget}} \\
\midrule
\textbf{Method} & \textbf{ROUGE~\textuparrow} & \textbf{Prob~\textuparrow} & \textbf{Truth Ratio~\textuparrow} \\
\midrule
\rowcolor{lightgray}  Baseline & 0.403 ± 0.017 & 0.230 ± 0.072 & 0.741 ± 0.023 \\
UCD & 0.360 ± 0.045 & 0.201 ± 0.050 & 0.679 ± 0.003 \\
\rowcolor{lightgray}  UCS & 0.596 ± 0.203 & 0.490 ± 0.348 & 0.638 ± 0.028 \\
Grad Ascent & 0.221 ± 0.241 & 0.072 ± 0.079 & 0.736 ± 0.029 \\
\rowcolor{lightgray}  Grad Diff & 0.004 ± 0.001 & 0.000 ± 0.000 & 0.732 ± 0.005 \\
NPO & 0.357 ± 0.088 & 0.114 ± 0.044 & 0.719 ± 0.019 \\
\rowcolor{lightgray}  NPO + RT & 0.281 ± 0.023 & 0.051 ± 0.002 & 0.701 ± 0.005 \\
\bottomrule
\end{tabular}
\caption{Additional metrics comparing baselines and UCD / UCS on Llama2-13B from TOFU 10\% measuring model utility on the forget QA pairs.}
\end{table}

==> qjbrrrnydnfnmpfdqhfjznfbtydkxrnq/macros.tex <==
\usepackage{multirow,nicefrac}

\usepackage[most]{tcolorbox} 
\PassOptionsToPackage{table}{xcolor}
\usepackage{xcolor}
\usepackage{colortbl}

\definecolor{lightgray}{gray}{0.9}  %
\definecolor{llamacol}{rgb}{0.19, 0.55, 0.91}
\definecolor{mistralcol}{rgb}{0.93, 0.53, 0.18}
\definecolor{phicol}{rgb}{0.31, 0.78, 0.47}

\usepackage{longtable}
\renewcommand{\arraystretch}{1.25}
% Adjust spacing around rules (set to 0pt to remove space)
% \setlength{\aboverulesep}{0pt}
\setlength{\belowrulesep}{0pt}




\newcommand{\promptbox}[1]{
\begin{tcolorbox}[colback=gray!10, colframe=black, rounded corners, boxrule=0.6mm, 
                  title={}, fonttitle=\bfseries]
\textbf{\underline{Input Prompt}}: \vspace{2mm} \newline \texttt{#1}
\end{tcolorbox}
}



% Customizing the line style to be dotted
\tikzset{
  dotted_line/.style={dash pattern=on 1pt off 4pt, line width=0.5pt}
}


% \newcommand{\mistralbox}[3]{
% \begin{tcolorbox}[title=\textbf{Input Prompt:} , breakable, enhanced, colframe=black, colback=mistralcol!10!white, coltitle=black, colbacktitle=mistralcol!50!white, boxrule=0.4mm, fonttitle=\bfseries]
% {\textbf{\underline{Base Model}:} #1}
%   \tcbline % Inserts a dotted line
% {\textbf{\underline{UCD Model}:} #2}
%   \tcbline % Inserts a dotted line
% {\textbf{\underline{Retrained from Scratch Model}:} #3}
% \end{tcolorbox}
% } 



\newcommand{\llamabox}[2]{
\begin{tcolorbox}[title=$\llama~\gen$, breakable, enhanced, colframe=black, breakable, colback=llamacol!10!white,  boxrule=0.4mm, coltitle=black, colbacktitle=llamacol!50!white, fonttitle=\bfseries]
{\textbf{\underline{Base Model}:} #1}
\tcblower 
{\textbf{\underline{Watermarked Model}:} #2}
\end{tcolorbox}
}

\newcommand{\phibox}[2]{
\begin{tcolorbox}[title= $\phimini~\gen$, breakable, enhanced,   colframe=black,  boxrule=0.4mm, colback=phicol!10!white, coltitle=black, colbacktitle=phicol!50!white, fonttitle=\bfseries, enlarge bottom by=2mm] 
{\textbf{\underline{Base Model}:} #1}
\tcblower 
{\textbf{\underline{Watermarked Model}:} #2}
\end{tcolorbox}
}




%% Different Models 
\newcommand{\smg}{\mathrm{A}_{\mathrm{clean}}}
\newcommand{\smb}{\mathrm{A}_{\mathrm{corr}}} 
\newcommand{\lmg}{\mathrm{P}_{\mathrm{clean}}}

\newcommand{\lma}{\mathrm{P}_{\mathrm{aligned}}}

\newcommand{\lmb}{\mathrm{P}_{\mathrm{corr}}}   


==> qjbrrrnydnfnmpfdqhfjznfbtydkxrnq/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak





==> qjbrrrnydnfnmpfdqhfjznfbtydkxrnq/plan.tex <==

\vmscomment{TODO LIST for Vinith: 1. Section 5 writing and plots
2. Section 6 writing and plots
3. Difference correlation analysis for approximation assumption, 4. Section 7, 5. Figure 1 -- visualization of contrastive decoding, 6. Appendix
    1. Sampling plots for TOFU
    2. Table with Probability, ROUGE-L, and Truth Ratio for TOFU
    3. Example Generations
        1. TOFU 10%
}


==> qjbrrrnydnfnmpfdqhfjznfbtydkxrnq/problem_setup.tex <==
\paragraph{Gradient Ascent (GA)} A common unlearning baseline, GA maximizes the next-token prediction loss on the forget set to reverse learning on those examples: \begin{equation*} \mathcal{L}{\texttt{GA}} = \mathbb{E}{x\sim\mathcal{D}_{\texttt{forget}}}[\log(\pi(y|x))] \end{equation*} While simple and direct, GA often serves as the foundation for more stable and effective variants.

\paragraph{Gradient Difference (GD)} Extends GA by adding a standard training loss on the retain set to preserve performance: \begin{equation*} \mathcal{L}{\texttt{GD}} = -\mathbb{E}{x\sim\mathcal{D}{\texttt{forget}}}[\log(\pi(y|x))] + \mathbb{E}{x\sim\mathcal{D}_{\texttt{retain}}}[\log(\pi(y|x))]
\end{equation*}

\paragraph{KL Regularization} Adds a KL term to control divergence between the updated model and a reference model on either the forget or retain set: \begin{equation*} \mathcal{L}{\texttt{KL}}(\pi,\refmodel) = \mathbb{E}{x\sim\mathcal{D}{\texttt{choice}}}[D{\texttt{KL}}(\pi(y|x)|\refmodel(y|x))], \quad \texttt{choice} \in {\texttt{forget}, \texttt{retain}} \end{equation*} This encourages forgetting via divergence on $\mathcal{D}{\texttt{forget}}$ or stability via alignment on $\mathcal{D}{\texttt{retain}}$.

\paragraph{Preference Optimization (PO)} Optimizes for refusal-like or random responses on the forget set while retaining standard performance elsewhere: \begin{equation*} \mathcal{L}{\texttt{PO}} = \mathbb{E}{x\sim\mathcal{D}{\texttt{alt}}}[\log(\pi(y|x))] + \mathbb{E}{x\sim\mathcal{D}{\texttt{retain}}}[\log(\pi(y|x))] \end{equation*} Here, $\mathcal{D}{\texttt{alt}}$ may include modified forget samples with refusal or random targets.

\paragraph{Negative Preference Optimization (NPO)} Adapts Direct Preference Optimization by treating the forget set as a negative-only preference dataset. The resulting objective is: \begin{equation*} \mathcal{L}{\texttt{NPO}} = \frac{2}{\beta}\mathbb{E}{x\sim\mathcal{D}{\texttt{forget}}}\left[\log\left(1 + \left(\frac{\pi{\theta}(y|x)}{\refmodel(y|x)}\right)^{\beta}\right)\right] \end{equation*}
